Conjunctive Queries with Theta Joins Under Updates

Modern application domains such as Composite Event Recognition (CER) and real-time Analytics require the ability to dynamically refresh query results under high update rates. Traditional approaches to this problem are based either on the materialization of subresults (to avoid their recomputation) or on the recomputation of subresults (to avoid the space overhead of materialization). Both techniques have recently been shown suboptimal: instead of materializing results and subresults, one can maintain a data structure that supports efficient maintenance under updates and can quickly enumerate the full query output, as well as the changes produced under single updates. Unfortunately, these data structures have been developed only for aggregate-join queries composed of equi-joins, limiting their applicability in domains such as CER where temporal joins are commonplace. In this paper, we present a new approach for dynamically evaluating queries with multi-way theta-joins under updates that is effective in avoiding both materialization and recomputation of results, while supporting a wide range of applications. To do this we generalize Dynamic Yannakakis, an algorithm for dynamically processing acyclic equi-join queries. In tandem, and of independent interest, we generalize the notions of acyclicity and free-connexity to arbitrary theta-joins and show how to compute corresponding join trees. We instantiate our framework to the case where theta-joins are only composed of equalities and inequalities and experimentally compare our algorithm to state of the art CER systems as well as incremental view maintenance engines. Our approach performs consistently better than the competitor systems with up to two orders of magnitude improvements in both time and memory consumption.

==> sections/relatedwork.tex <==
%!TEX root = ../main/main.tex

\paragraph*
{Incremental View Maintenance} The problem of
incrementally maintaining materialized answers to conjunctive queries
under updates has been extensively studied. We refer to
\cite{gupt-materializedviews-book,DBLP:journals/ftdb/ChirkovaY12} for an overview. Our work
differs from traditional IVM in that we maintain data structures that do not fully
materialize query results.
 In addition, we support queries with
multi-way $\theta$-joins. 

% In the equi-join setting, Nikolic and
% Olteanu have recently proposed IVM methods based on
% factorization. On free-connex acyclic \cqs, this method is equivalent
% to \dyn. While \cqs that are not free-connex acyclic are also
% supported by their method, such queries require more than linear
% storage space, or less-efficient update times. 


\paragraph*
{Constant Delay Enumeration} There is increasing work
on query evaluation with constant-delay
enumeration~\cite{Bagan:2007,DBLP:journals/sigmod/Segoufin15,Berkholz:2017,braultbaron,Olteanu:2015,Bakibayev:2013,Olteanu:2015,Schleich:2016,dyn:2017,DBLP:conf/pods/FlorenzanoRUVV18}. Similar
to \dyn, \edyn, and \iedyn, these works separate query processing in a
processing stage and an enumeration phase and guarantee that, during
enumeration, only a constant amount of work is required to produce
each new result tuple. In contrast to \edyn and \iedyn, however, they
focus on the static setting and deal with equi-joins only.

\paragraph*
{Algorithms for processing inequality joins} In the static setting,
common ways to evaluate an inequality join between two relations
include variants of sort-merge and partition
joins~\cite{DBLP:conf/vldb/DeWittNS91}, as well as index joins using
interval-based
indexing~\cite{DBLP:conf/vldb/HellersteinNP95,DBLP:conf/sigmod/EnderleHS04}. Our
work, in contrast, considers dynamic processing of multi-way
inequality and 
$\theta$-joins. We leverage the sort-merge inequality join as a
building block. Recently, Khayyat et
al.~\cite{DBLP:journals/vldb/KhayyatLSOPQ0K17} have proposed fast
multi-way inequality join algorithms based on sorted arrays and space
efficient bit-arrays. They focus on the case where there are exactly
two inequality conditions per pairwise join. While they also present
an incremental algorithm for pairwise joins, their algorithm does not
consider constant delay enumeration and makes no effort to minimize
the update cost in the case of multi-way joins. As a result, in that
case, they need to either materialize subresults (implying a
space-overhead that is potentially more than linear), or recompute
subresults. We do neither.


\paragraph*{\cer} There is a multitude of research on Composite
Event Recognition (\cer); we refer to
\cite{cugola:2012,DBLP:conf/debs/ArtikisMUVW17} for a survey. An
important direction in \cer research is the design of declarative
languages for specifying \cer patterns. Our work, in contrast, focuses
on the dynamic execution of multi-way $\theta$-joins, which naturally
occur in \cer \textsf{SEQ} patterns (exemplified by the fraud
query). We experimentally compare against multiple state-of the art
\cer engines in Section~\ref{sec:experiments}.

\newcommand{\semijoinprog}{\ensuremath{\mathcal{S}}}
\paragraph*{Acyclicity} The notion of ayclicity is well-studied in
database theory~\cite{abiteboul1995foundations} due to the fact that
acyclic \cqs can be evaluated in time that is linear in both the input
and output, and this under combined complexity. There are many equivalent ways of defining acyclicity for
standard \cqs, including by means of the \gyo reduction,
$\alpha$-acyclicity for hypergraphs, the existence of a standard join
tree\footnote{Not to be confused with the \gjts defined in this
  paper}, and the existence of a \emph{full reducer}. Here, a full
reducer for a \cq $Q$ is a program $\semijoinprog$ in the semijoin
algebra (the variant of relational algebra where joins are replaced by
semijoins) that, given a database $\db$ computes a new database
$\semijoinprog(\db)$ with the following properties. (1)
$Q(\semijoinprog(\db)) = Q(\db)$. (2) and
$\semijoinprog(\db)_{r(\seq{x})} \subseteq \db_{r(\seq{x})}$ for every
atom $r(\seq{x})$ in $Q$; and (3) no strict subset of
$\semijoinprog(\db)$ has $Q(\semijoinprog(\db)) = Q(\db)$. In other
words, $\semijoinprog(\db)$ selects a \emph{minimal} subset of $\db$
needed to answer $Q$.

Bernstein and Goodman~\cite{DBLP:journals/is/BernsteinG81} consider
conjunctive queries with inequalities and classify the class of such
queries that admit full reducers. As such, one can view this as a
definition of acyclicity for conjunctive queries with
inequalities. Bernstein and Goodman's notion of acyclicity is
incomparable to ours. On the on hand, our definition is more general:
Bernstein and Goodman consider only queries where for each pair of
atoms there is exactly one variable being compared by means of
equality or inequality. We, in contrast, allow an arbitrary number of
variables to be compared per pair of atoms. In particular, Bernstein
and Goodman's disallow queries like $(r(x,y), s(x,z) \mid y < z)$
since it compares $r.x$ with $s.x$ by means of equality and $r.y <
s.z$ by means of inequality.

On the other hand, for this more restricted class of queries,
Bernstein and Goodman show that certain queries that we consider to be
cyclic have full reducers (and would be hence acyclic under their
notion). An example here is
\begin{multline*}
 r(x_r) \Join s(x_s,
y_s) \Join t(x_t, y_t) \Join u(y_u) \\ \mid x_s \leq x_r, x_t \leq x_r,
y_s \leq y_u, y_t \leq y_u 
\end{multline*}
The crucial reason that this query admits a full reducer is due to the
transitivity of $\leq$. Since our notion of acyclicity interprets
predicates abstractly and does hence not assume properties such as
transitivity on them, we must declare this query cyclic. It is an
interesting direction for future work to incorporate Bernstein and
Goodman's notion of acyclicity in our framework.






%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../main/main"
%%% End: 

